A Review of Conceptualizations of Safety and Risk in Current Automated Driving Regulation

"Safety" and "Risk" are key concepts for the design and development of automated vehicles. For the market introduction or large-scale field tests, both concepts are not only relevant for engineers developing the vehicles, but for all stakeholders (e.g., regulators, lawyers, or the general public) who have stakes in the technology. In the communication between stakeholder groups, common notions of these abstract concepts are key for efficient communication and setting mutual expectations. In the European market, automated vehicles require Europe-wide type approval or at least operating permits in the individual states. For this, a central means of communication between regulators and engineers are regulatory documents. Flawed terminology regarding the safety expectations for automated vehicles can unnecessarily complicate relations between regulators and manufacturers, and thus hinder the introduction of the technology. In this paper, we review relevant documents at the UN- and EU-level, for the UK, and Germany regarding their (implied) notions of safety and risk. We contrast the regulatory notions with established and more recently developing notions of safety and risk in the field of automated driving. Based on the analysis, we provide recommendations on how explicit definitions of safety and risk in regulatory documents can support rather than hinder the market introduction of automated vehicles.

==> macros.tex <==
% macros for file path handling
\makeatletter
\newcommand{\getfileext}[1]{%
	\filename@parse{#1}
	\def\thefileext{\filename@ext}
}
\makeatother

% enable column equalization with biblatex
\makeatletter
\newcounter{IEEE@bibentries}
\renewcommand\IEEEtriggeratref[1]{%
	\renewbibmacro{finentry}{%
		\stepcounter{IEEE@bibentries}%
		\ifthenelse{\equal{\value{IEEE@bibentries}}{#1}}
		{\finentry\@IEEEtriggercmd}
		{\finentry}%
	}%
}
\makeatother

%copyrightnotice IEEE with tikz
\ifx \isaccepted \undefined
\newcommand\copyrighttext{%
	\footnotesize \centering This work has been submitted to the IEEE for possible publication.\\ Copyright may be transferred without notice, after which this version may no longer be accessible.}
\else
\newcommand\copyrighttext{%
	\footnotesize \parbox[t]{.11\textwidth}{\copyright{} \the\year~IEEE.} \parbox[t]{.89\textwidth}{Personal use of this material is permitted. Permission from IEEE must be obtained for all other uses, in any current or future media, including reprinting/republishing this material for advertising or promotional purposes, creating new collective works, for resale or redistribution to servers or lists, or reuse of any copyrighted component of this work in other works.}}
\fi
\newcommand\copyrightnotice{%
	\ifx \compileforpublish \undefined
	\else
	\begin{tikzpicture}[remember picture,overlay]
	\node[anchor=south,yshift=10.5pt] at (current page.south) {\parbox{\dimexpr\textwidth-\fboxsep-\fboxrule\relax}{\copyrighttext}};
	\end{tikzpicture}%
	\fi
}



\newcommand{\comment}[2][]{\textcolor{#1}{\uppercase{#1}: #2}} 
\newenvironment{oldtext}{\par\color{gray}}{\par}
%\usepackage{comment}
%\excludecomment{oldtext}
\newcommand{\estmat}[1]{\hat{\mathbf{#1}}}
\newcommand{\vect}[1]{\mathbf{#1}}

\newcommand{\todo}[1]{\emph{\textcolor{red}{(TODO: #1)}}}

%% some file path handling magic: we want to automatically include images, given that the document tex file structre is mirrored in a figures/images/vector /raster or /tikz folder
% e.g. to include a file by using \includeimg{myfile} instead of \includegraphics{figures/images/vector/01_motivation/02_cool_motivation/myfile.pdf}


\tikzset{external/system call={pdflatex -enable-write18 -halt-on-error
		-interaction=batchmode -jobname "\image" "\texsource" -aux-directory=\currfileabsdir/auxfiles_tikz}}

\graphicspath{{figures/images/tikz/}{figures/images/raster/}{figures/images/vector/}}
\svgpath{figures/images/vector/svg/}

\newcommand{\getimgpath}{%
	\StrBehind{\currfiledir}{/}[\imgbase]%
}

% in order to use xstring's \StrSubstitute with currfile, we must get rid of backslashes, converting a backslash to a decent catcode is a pain -> verbtocs does this for us.
\verbtocs{\bs} |\|

% get current tex file's directory
\newcommand{\getfilepathbs}{%
	\StrSubstitute{\detokenize{\currfiledir}}{\bs}{/}[\thefilepathbs]%
}

% get relative desired image path based on tex file's path
\newcommand{\getrelimgpath}{%
	\getfilepathbs
	\StrBehind*{\thefilepathbs}{content/}[\relimgpath]%
}

\newcommand{\getfilebasename}[1]{%
	\StrBefore*{#1}{.}[\thefilebasename]
}

\newcommand{\getimglastdir}{%
	\getfilepathbs%
	\StrGobbleRight{\thefilepathbs}{1}[\gobbled]%
	\StrCount{\gobbled}{/}[\numSlashes]%
	\StrBehind*[\numSlashes]{\gobbled}{content/}[\imglastdir]%
}


% use relative image path to move externalized tikz files to a directory where only vector files are located
\newcommand{\mytikzexternalenable}{%
	\getrelimgpath%
	\tikzsetexternalprefix{figures/images/vector/\relimgpath}%
	\tikzexternalenable%
}

% macro to include tikz files

%define option keys
\pgfkeys{
	/inputtikz/.is family, /inputtikz,
	depends/.estore in = \tikzIsDependendOn,
	externalize/.estore in = \tikzShallExternalize,
	width/.estore in = \tikzPicWidth
}
\options{%
	/inputtikz/.new family,
	/inputtikz/depends/.new value=[]{},
	/inputtikz/externalize/.new value=[false]{false},
	/inputtikz/width/.new value,
}
\newcommand{\inputtikz}[2][]{%
	\getrelimgpath%
	{\options{/inputtikz, #1}%
	\ifoptionvoid{/inputtikz/depends}{%
	}{%
		\ifoptionblank{/inputtikz/depends}{%
		}{%
			\tikzpicturedependsonfile{\option{/inputtikz/depends}}%
		}%
	}%
	%
	\ifoptionvoid{/inputtikz/width}{%
	}{%
		\ifoptionblank{/inputtikz/width}{%
		}{%
			\begin{adjustbox}{width=\option{/inputtikz/width}}
		}%
	}%	
	\ifoptionequal{/inputtikz/externalize}{true}{%
		\getfilebasename{#2}%
		\newcommand{\myfilebase}{\thefilebasename}%
		\tikzsetfigurename{\myfilebase}%
		\mytikzexternalenable%
		\input{figures/images/tikz/\relimgpath#2}%
		\tikzexternaldisable%
	}{%
		\input{figures/images/tikz/\relimgpath#2}%
	}%
	\ifoptionvoid{/inputtikz/width}{%
	}{%
		\ifoptionblank{/inputtikz/width}{%
		}{%
			\end{adjustbox}
		}%
	}}%
}%
\makeatletter
\newcommand\notsotiny{\@setfontsize\notsotiny{6.5}{7.5}}
\makeatother

\newcommand{\includeimg}[2][]{%
	\getfileext{#2}
	{\options{/inputtikz, #1}
		\IfSubStr{\thefileext}{tikz}{%
			\getimgpath%
			\IfSubStr*{\currfileext}{tikz}{\StrBehind*{\imgbase}{images/tikz/}[\imgbase]}{}%
			\inputtikz[#1]{\imgbase#2}
		}{%
            \IfSubStr{\thefileext}{svg}{%
			\getimgpath%
			\IfSubStr*{\currfileext}{tikz}{\StrBehind*{\imgbase}{images/tikz/}[\imgbase]}{}%
			 \escapeus{\includesvg[pretex=\notsotiny, #1]{\imgbase#2}}%
		  }{%
			\getimgpath%
			\IfSubStr*{\currfileext}{tikz}{\StrBehind*{\imgbase}{images/tikz/}[\imgbase]}{}%
			\IfSubStr*{\thefileext}{table}{%
				\input{tables/\imgbase#2}
			}%
			{%
				\IfSubStr*{\currfileext}{tikz}{\StrBehind*{\imgbase}{images/tikz/}[\imgbase]}{}%
				\includegraphics[#1]{\imgbase#2}%
			}%
        }%
	}}%
}%


==> tools/README <==

August 26, 2015


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. The \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later.

 3. The \IEEEnoauxwrite command.

 4. The IEEE itemize, enumerate and description list environments.

 5. The complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 6. The \IEEEQEDhere and \IEEEQEDhereams commands to provide amsthm.sty
    \qedhere functionality to IEEEproof. \IEEEQEDhere is for simple use
    "right on the spot" such as within an IEEEeqnarry:

    \begin{IEEEproof}
       \begin{IEEEeqnarray}{rCl+x*}
        x & = & y & \nonumber\IEEEQEDhere
       \end{IEEEeqnarray}
    \end{IEEEproof}

    While \IEEEQEDhereams is like amsthm's venerable \qedhere and is
    for use within the standard equation environment:

    \begin{IEEEproof}
     \begin{equation}
       x = y \nonumber\IEEEQEDhereams\quad
     \end{equation}
    \end{IEEEproof}

    Note that the qedhere style is normally not done with IEEE-related
    work so these are undocumented features of IEEEtran.cls.

    Thanks Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser for
    suggesting this feature.



IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
2015/08/26 V1.5 (V1.8b of IEEEtran.cls) changes:

 1) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 2) Fix bug with IEEEeqnarray equation number foreground color
    under the color environment of Beamer class.
    Thanks to Joschi Brauchle for reporting this problem.

 3) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.



********************************** Files **********************************

README                - This file.

changelog.txt         - The revision history.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************


